Technical Report: Assisting Backdoor Federated Learning with Whole Population Knowledge Alignment

Due to the distributed nature of Federated Learning (FL), researchers have uncovered that FL is vulnerable to backdoor attacks, which aim at injecting a sub-task into the FL without corrupting the performance of the main task. Single-shot backdoor attack achieves high accuracy on both the main task and backdoor sub-task when injected at the FL model convergence. However, the early-injected single-shot backdoor attack is ineffective because: (1) the maximum backdoor effectiveness is not reached at injection because of the dilution effect from normal local updates; (2) the backdoor effect decreases quickly as the backdoor will be overwritten by the newcoming normal local updates. In this paper, we strengthen the early-injected single-shot backdoor attack utilizing FL model information leakage. We show that the FL convergence can be expedited if the client trains on a dataset that mimics the distribution and gradients of the whole population. Based on this observation, we proposed a two-phase backdoor attack, which includes a preliminary phase for the subsequent backdoor attack. In the preliminary phase, the attacker-controlled client first launches a whole population distribution inference attack and then trains on a locally crafted dataset that is aligned with both the gradient and inferred distribution. Benefiting from the preliminary phase, the later injected backdoor achieves better effectiveness as the backdoor effect will be less likely to be diluted by the normal model updates. Extensive experiments are conducted on MNIST dataset under various data heterogeneity settings to evaluate the effectiveness of the proposed backdoor attack. Results show that the proposed backdoor outperforms existing backdoor attacks in both success rate and longevity, even when defense mechanisms are in place.

==> useless.tex <==
% weight divergence between a centralized learning model (CL) and FL global model in one specific FL aggregation and find that a client's weight divergence is only caused by the label distribution (henceforth referred to as ``distribution") and gradient difference between the local data and the aggregation of the global data, namely the whole population of all clients' data. 

%  In particular, based on the findings in \cite{xu2020federated}, we further analyze the Based on this observation, a client can alleviate the weight divergence by training on a crafted local dataset, which mimics the distribution of the global data. 

% In the preliminary phase, the attacker does not take any malicious backdoor action. 
% difference to existing studies.
% 1. does not provides whole population information.
% 2. does not produce a quantitative property of the dataset.
% The proposed two-phase backdoor attack presents the following two features: 
% (1) Existing backdoor attacks do not interfere the training process. In contrast, in our proposed attack, our backdoor attacks participate in the training process by the malicious clients training on crafted dataset that aligns with the inferred global distribution. In this case, the alleviated weight divergence improves the FL model accuracy, which earns a lengthened attack window for the backdoor injections. 
% (2) The proposed global data distribution inference attack is optimization-based, which produces precise quantitative property information about the dataset. In contrast, most of the property inference attacks can only cover limited number of pre-defined properties or qualitative information about the dataset. E.g., in \cite{ganju2018property, melis2019exploiting}, scholars proposed classifiers to infer if the training data has or has not the specific property , and a comparison method is proposed to infer which label has a larger size of  data samples \cite{wang2019eavesdrop}.

% Our proposed attack differentiates from the previous attacks in two ways. First, our attack targets on the property information about the whole population data, whereas the previous works focus on the information about the individual data sample. Secondly, our attack is formulated as an optimization problem in the continuous space, in which the solution is a vector of continuous values. On the contrary, the existing property inference attacks are classifier-based, which can only cover limited number of pre-defined properties. 

% The global label distribution is estimated, in which the distance between the FL model updates and the updates composed by the estimated global label distribution and the gradients is minimized.

% \item We propose a two-phase backdoor attack, which expedite the FL model early stage convergence behavior by aligning, so as to increase the success rate and longevity of early-injected backdoor attack. 

% \item Based on the findings in \citep{xu2020federated}, we prove the weight divergence of the FL local model and the CL model within one FL aggregation is positively to the label distribution distance as well as the gradient distance calculated over local data and global data. We show that the FL convergence can be facilitated if client reduce such two distances.


 Therefore it is assumed that the central server is unable to validate the legitimacy of the received model updates. This gives adversaries enough space to manipulate the data or poison the model without being recognized.
 
 
 


 For example, As stated by scholars in \citep{chase2021property}, property inference attacks could pose negative impact on governments and companies. As already in used applications, such as spam classifier, fraud detector and etc. could leak sensitive information about the clients and transactions. 
 
 
 
However, backdoor injections in the early training stage can be erased quickly by the new benign model updates, as the model updates contain more clients' shared information rather than individual features at this point. We show the FL accuracy can be alleviated by aligning the local data distribution with the inferred global data distribution. The improved training accuracy provides the backdoor a lengthened attack window.

Further, while these methods are effective in defending against single-shot backdoor attacks, they are not as effective in defending against multi-shot backdoor attacks. To account for the model updates from non-i.i.d clients, most of the methods do not differentiate malicious model updates from benign ones or the estimated mean and kick them out. Instead, they aim to mitigate their negative impacts by assigning a smaller weight when aggregating on the server. These mechanisms easily mitigate the effect of the single-shot backdoor attack. However, multiple-shot backdoor attacks could still reach a high success rate \cite{}. When continuously injecting the backdoored model updates, there is an iterative and amplified effect of the injected backdoors, that is part of the previously injected backdoor is integrated in the global model aggregation, making the later injected backdoors have a higher chance to be assigned with a larger weight. 



 we take one step further. We want to get rid of the accumulated effect from previous aggregations and are more interested in the weight divergence of $w_{cen}$ and $w_{fl}$, and $w_{cen}$ and $w_k$ between two FL global aggregations. T 


These two differences contributing to the weight divergence, are also the main cause of the slower convergence and accuracy degradation in FL, compared to the centralized learning.

Specifically, in the preliminary phase, the attacker first infers the label composition of the whole population data and then constructs an auxiliary dataset that aligns with the inferred label composition. The procedure alleviates the weight divergence and improves the FL model accuracy, providing benefits for the later backdoor injections. Then, the backdoors are injected at the global model convergence or when a specific accuracy is met. 

reduce the weight divergence by inferring the whole population label distribution and training on crafted auxiliary datasets that align with the inferred distribution. 
Given the fact that the backdoor injected close to the FL model convergence is more likely to survive, the assistance phase serves as a role to improve the main task accuracy in the early training stage. To achieve the goal of improving FL model main task accuracy, the compromised clients mimic the behavior of a CL process. 

When an expected FL model accuracy or the convergence is reached, the attacker launches the backdoor attack by training on the backdoored dataset. Each training batch is a mix of clean data and backdoored data. 

Since the central server aggregates multiple model updates to update the global model, the contribution of the backdoored model to the global model could be very limited. Before sending to the server, the backdoored model update is scaled by $\gamma = K$ 

Recall that the goal of the attacker is to find an estimation of the whole population label composition $p(y)$, denoted as $\hat{p}(y)$.  Since attacker has no access to the losses of other clients, nor the global loss, this solution does not directly apply. Fortunately, 

We set $\theta=0.8$, in which a greater $\theta$ indicates greater estimation precision and greater augmentations.

Note that the difference between the existing backdoor attacks and our proposed backdoor attack lies in  that our proposed backdoor attack utilizes the information leakage to make the injected backdoor more persistent. As mentioned previously, the single-shot backdoor is better to inject when the global model accuracy is relatively high, to reach its maximum effectiveness (in both attack success rate and longevity).


the attacker submit the model weight update that is generated on the auxiliary dataset to facilitate the training process. The adversary will not inject the backdoor until a desired global model accuracy is reaches. The completion of the backdoor injection happens without any involvement of the assistant clients.  When the attacker decides to inject a backdoor, the attacker poisons the local data $D_a$  



% randomness  
The experimental results are averaged over 10 experiments to eliminate the impact of randomness.


    As the adversary needs to fine-tune the local training parameters, such as the internal epoch and the local learning rate, to reach the maximum effectiveness of the backdoor attack. However, the success and the stealthiness of the backdoor injection are usually brought by a smaller learning rate and more internal training epochs compared to those of a benign training, which could result in a sudden increase in the main-task accuracy. Such an unexpected increase in the main-task could alert the server about the security of the local model updates. 
    
    The method evaluates the amount of the augmentations by measuring the directional distance between the gradient of the augmentation and the expected gradients. A scaler $\theta \in [0, 1]$, indicating the \textit{cosine similarity} of the gradients on the augmentations and the expected gradient, is used to determine the precision of the estimation and the amount of augmentation. 
    
    In addition, the global distribution alignment has more influence on the early stage training performance (epoch 0 to epoch 15) as the local data becomes more non-i.i.d. 
    
    
    s evidenced in setting 2 and setting 4 in Fig. \ref{convergence}, where the local data distributions are more non-i.i.d ($\alpha=0.1$), the convergence performance gain by the distribution alignment is more visible in the middle training stage (epoch 10 to 20) compared to the Setting 1 and Setting 3 ($\alpha=1$), in which the improvement of convergence lies in the early stage (epoch 0 to 10).
    
    
    
    \textbf{Global knowledge alignment improves the main-task accuracy at the early training stage} We evaluate the FL model accuracy with the assistance of global distribution alignment, i.e., the accuracy gain obtained by the preliminary phase of the proposed backdoor attack, shown in Fig. ~\ref{convergence}. The clients are randomly selected to participate in a round of training. For a fair comparison, the total data size of $D_{aux}$ is the same as that of the original dataset $D_a$. The "regular FL" refers to the conventional FL training without the assistance of global distribution alignment, where as "aux\_5", "aux\_10" and "aux\_20" denote the percentages of the compromised clients to be $5\%$, $10\%$ and $20\%$ of the total number of clients, respectively.

In general, the accuracy with the assistance of global distribution alignment is higher than the baseline accuracy. Higher percentage of malicious clients leads to a greater gain in the main-task accuracy, compared to the baseline. In addition, the global distribution alignment has more influence on the early stage training performance as the local data becomes more non-i.i.d. As evidenced in settings 2 and 4 in Fig. \ref{convergence}, where the local data distribution is highly non-i.i.d, the main-task accuracy reaches a higher value compared to that of the baseline. The experimental results match the findings in Proposition 1 in the paper: when the local data distributions are non-i.i.d, aligning the local distribution with the global distribution could increase the FL training accuracy.


We evaluate the proposed two-phase backdoor and compare our approach with two existing backdoor attacks: (1) the centralized backdoor attack in \cite{bagdasaryan2018backdoor} (referred to as ``baseline''), in which the local dataset is poisoned by a centralized backdoor trigger; (2) the distributed backdoor attack \citep{xie2019dba} (referred to as DBA), in which the backdoor trigger is partitioned and each part of the backdoor is injected separately. 

We compare the proposed two-phase backdoor with the ones proposed in \cite{bagdasaryan2018backdoor} (referred to as ``baseline'') and \cite{xie2019dba} (referred to as``DBA'') and the proposed two-phase backdoor attack, shown in Fig. \ref{fig::main_task_acc}. In our proposed backdoor attack, "aux\_5", "aux\_10" and "aux\_20" denote the percentages of the compromised clients to be $5\%$, $10\%$ and $20\%$ of the total number of clients, respectively.



% It is claimed in \citep{xie2019dba} that DBA splitting and distributing the backdoor trigger in to several clients could increase the stealthiness of the injected backdoor, however, the sudden leap in the main-task accuracy could alarm the central server about the presence of malicious model updates. Meanwhile, both backdoor injection against regular FL (baseline) and our proposed whole population knowledge assisted FL drop the main-task accuracy at time of injection. But the main-task accuracy drop in our proposed FL is less perceptible than that of the baseline FL, which indicates the proposed whole population assisted FL makes the backdoor injection more stealthy than the baseline FL. 

a  the effectiveness of the single-shot backdoor increases when being injected in later training rounds.

since the most favorable scenario for backdoor injection is when FL global model reaches a high accuracy, indicating the local model updates become similar and begin to cancel out \cite{bagdasaryan2018backdoor}.

We investigate the computational complexity of the proposed inference attack to see if it is feasible to mount such an inference attack on a FL client. 

Batch gradient has a time complexity of $\mathcal{O}(n^2 m)$, in which $n$ is the number of data samples and $m$ is the number of features. 

% Single-shot backdoor attacks rely on the scaling operation to achieve the goal of global model replacement, hence are easier to detect and hardly succeed when defense strategies are in the place. Therefore, we will focus on evaluating the attack effectiveness of the proposed backdoor and the ``baseline'', and ``DBA'' against both FoolsGold and DP under multi-shot backdoor settings.

intentionally protects the privacy, but in theory, they can be used to defend against backdoor attacks. DP 

While this method is not meant to provide privacy, in practice, they do not defend against inference attacks. Authors in [] stated that DP could mitigate both backdoor and inference attacks. 


The effect of malicious model updates can also be reduced. Because the backdoor attack increases the distance of the backdoored model updates to benign model updates, the efficacy of the backdoor can be reduced by the clipping bound. 

% calculates the cosine similarity across the model updates and de-emphasizes the model updates that are similar to each other, it could unintentionally discard lso reduces the effect of non-i.i.d. distribution among clients, making the inference about the global data distribution even more accurate.  

, leading to a reduced combined effectiveness as well as a faster diminish rate. 
% Our experiments show that DP does defend against backdoor attacks even with a large privacy budget (smaller noise scale). And it is more effective than the FoolsGold defense strategy.

% for 
% and the proposed backdoor have a similar pattern, where the success rate reaches its maximum at the time of injection and then decreases as the training going on. I


We assume the attacker compromised clients play two roles, namely the assistant client and backdoor client. 

Even a large privacy budget, i.e., a small noise scale could drastically weaken the effectiveness of a backdoor attack. 

Again, purely pursuing a large size of the auxiliary dataset may introduce excessive computation
and similar samples, which could in turn be harmful to the FL global model.

% A high $\epsilon$ generating a large $\sigma$ could decrease both main-task and backdoor-task accuracy. The proposed attack still achieves $x\%$ backdoor accuracy. 
